FSD-Inference: Fully Serverless Distributed Inference with Scalable Cloud Communication

Serverless computing offers attractive scalability, elasticity and cost-effectiveness. However, constraints on memory, CPU and function runtime have hindered its adoption for data-intensive applications and machine learning (ML) workloads. Traditional 'server-ful' platforms enable distributed computation via fast networks and well-established inter-process communication (IPC) mechanisms such as MPI and shared memory. In the absence of such solutions in the serverless domain, parallel computation with significant IPC requirements is challenging. We present FSD-Inference, the first fully serverless and highly scalable system for distributed ML inference. We explore potential communication channels, in conjunction with Function-as-a-Service (FaaS) compute, to design a state-of-the-art solution for distributed ML within the context of serverless data-intensive computing. We introduce novel fully serverless communication schemes for ML inference workloads, leveraging both cloud-based publish-subscribe/queueing and object storage offerings. We demonstrate how publish-subscribe/queueing services can be adapted for FaaS IPC with comparable performance to object storage, while offering significantly reduced cost at high parallelism levels. We conduct in-depth experiments on benchmark DNNs of various sizes. The results show that when compared to server-based alternatives, FSD-Inference is significantly more cost-effective and scalable, and can even achieve competitive performance against optimized HPC solutions. Experiments also confirm that our serverless solution can handle large distributed workloads and leverage high degrees of FaaS parallelism.

==> algos/serverless-spff-sns_OLD.tex <==
\begin{algorithmic}[h]
\DontPrintSemicolon
\caption{SSpInf with SDS-Inf-Queue}
\label{alg:spff-sns}
% \begin{algorithmic}
% \vspace{5pt}
\KwIn{$x_m^0, \{W_m^k\}, \{Xsend_{m}^k\}, \{Xrecv_{m}^k\}$}
% NEED TO CHANGE TO JUST M IN XSEND AND XRECV I THINK


% \hrulefill\\
\ForAll(){FaaS workers $P_m$ \text{in parallel}}{
    \For{$k = 1, 2, \dots, L$}{
        \ForEach{$(P_n, \bar{x}_{mn}^{k-1}) \in Xsend_m^k$}{
        % \If{$\bar{x}_{mn}^{k-1} == \emptyset$}{
            % \text{DynamoDB write}$(k, m, n)$
            % \texttt{NoSQL.write((k,m), n)} \\
        % }
        % \Else{
            $\bar{x}^{k-1}_{mn} \gets $\texttt{ extract\_rows($x^{k-1}_m, \bar{x}^{k-1}_{mn}$)}\\
            $Xsend\_list_m^k \gets Xsend\_list_m^k \cup \{(P_m, \bar{x}_{mni}^{k-1}) \} $
        % }
        }
        \ForEach{b \in \texttt{populate\_batches}($Xsend\_list_m^k)$}{
            % \text{Non-blocking SNS publish($b$)}
            \texttt{topic-\{m\%10\}.publish\_batch(b)} \\
        }
        $z_m^k \gets W_m^kx_m^{k-1}$\\
        \While{$len(Xrecv_m^k) > 0$}{
            % $Xdynamo_m^k \gets \text{DynamoDB Poll} ((k, m))$
            % $Xnull_m^k \gets $ \texttt{NoSQL.read((k,m))} \\
            % \ForEach{$P_n \in Xnull_m^k$}{
            %     \If {$(P_n, \hat{x}^{k-1}_{nm}) \in Xrecv^k_m$}{
            %         $Xrecv^k_m \gets Xrecv^k_m / (P_n, \hat{x}^{k-1}_{nm})$
            %     }
            % }
            % $Xpoll_m^k \gets \text{SQS Poll} (Q_m)$\\
            $Xpoll_m^k \gets $ \texttt{queue-\{m\}.poll()}\\
            \ForEach{$(P_n, \hat{x}_{nmi}^{k-1}) \in Xpoll_m^k$}{
                $Xrecv\_list_{m}^k \gets Xrecv\_list_{m}^k \cup \hat{x}_{nmi}^{k-1}$\\
                \If {$Xrecv\_list_{m}^k[P_n] == Xrecv_{m}^k[P_n]$}{
                    $Xrecv_{m}^k \gets Xrecv_{m}^k / (P_n, \hat{x}_{nm}^{k-1})$ 
                }
            }
            \texttt{queue-\{m\}.delete($Xpoll_m^k$)}
        }
        \ForEach{$\hat{x}_{nm}^k \in Xrecv\_list_m^k$}{
            $z_m^k \gets z_m^k + W_m^k \hat{x}_{nm}^k$
        }
        $x_m^k = f(x_m^k)$
    }
    
    \texttt{barrier($P_{all}$)}\\
    \texttt{reduce($P_0, x_m^L$)}\\
}

\If{FaaS Worker $P_0$}{
    \Return $x^L$
}

% \end{algorithmic}
% Coordinate results
% \hrulefill\\
% \tcc{Increment parent's level to obtain current level.}
% \
\end{algorithmic}

==> old/2-communication.tex <==
\section{Serverless Inter-Process Communication}
\label{s:communication}

This section presents cloud service categories for inter-process communication (IPC) and hypergraph-based partitioning for parallelizing large DNNs.

\subsection{Serverless Communication}
\label{ss:serverless-communication-offerings}
There is no native and direct serverless FaaS-to-FaaS communication solution analogous to the mechanisms used in the HPC setting. 
% ; only some partially serverless solutions have been recently proposed \cite{Bohringer2022FMI}. 
Reasons for this include function isolation and fast container switching \cite{Agache2020Firecracker, Brooker2023LambdaContainers}. 
% , as well as FaaS being positioned for short-lived, standalone, stateless and event-driven processing, rather than for distributed data-intensive computation.
%Another reasonable explanation would be considerations around provider network bandwidth/security; the only supported direct communication between a FaaS instance and its invoker is currently via the request payload and subsequent FaaS response, which are both size-limited \footnote{https://docs.aws.amazon.com/lambda/latest/dg/gettingstarted-limits.html}, enabling the provider to easily manage bandwidth and throughput requirements in their FaaS-hosting data centers. Allowing direct FaaS-to-FaaS communication would present additional risk and unpredictability in this respect. 
% as well as possible considerations around provider network bandwidth/security. 
Hence, prior work on serverless data analytics and ML \cite{Jonas2017Occupy,Muller2020Lambada, Shankar2020NumPyWrenSLA, Perron2020} has typically used non-serverless components for communication. 
%has used either non-serverless components or distributed object storage as communication channels. 
We now discuss the service categories that can be considered as part of a fully serverless communication solution.


\subsubsection{Data Streaming Systems}
% KDS provides a high throughput, low latency data streaming solution. Considerations for the SDS-Inf use case include a hard limit on the number of concurrent consumers per stream (currently 20); a maximum payload per putRecords request of 1MiB; a limit of  5 getRecords requests per second per shard; limited autoscaling functionality; and a lack of inbuilt message filtering (without incorporating additional components).

% - Features: High throughput, low latency distributed event log. 
Data streaming solutions offer high throughput and low latency distributed event logs which can be processed in near-real time. For a serverless ML inference workload, parallel FaaS workers could act as both producers (publishing events to the stream), and consumers (retrieving items from the stream). A stream is usually partitioned in such a way that it can be distributed across multiple processing nodes. Commercial cloud data streaming offerings include AWS Kinesis Data Streams, Azure Event Hubs and Google Datastream. They typically impose restrictions on the number of concurrent consumers per stream, maximum payload size, and number of API calls per second \footnote{https://docs.aws.amazon.com/streams/latest/dev/service-sizes-and-limits.html} \footnote{https://learn.microsoft.com/en-us/azure/event-hubs/event-hubs-quotas} \footnote{https://cloud.google.com/datastream/docs/quotas}, all of which impact their suitability for use in a scalable ML inference system.

Cloud providers also offer extract-transform-load (ETL) solutions on streaming data. Transformation features offered include data disaggregation and filtering, key-based partitioning and data compression, all of which could potentially be beneficial for our use case. However, current commercial offerings (e.g. AWS Kinesis Data Firehose) have large minimum buffer sizes (both in terms of data volume and time triggers), and are not directly pollable by consumers. Hence for our use case, while producers could directly publish messages to the ETL delivery stream, the buffered output would need to be written to an intermediate destination such as object storage, where FaaS consumers could then retrieve it.


% *cite AWS docs, Azure Docs (https://learn.microsoft.com/en-us/azure/event-hubs/event-hubs-quotas), Google docs (https://cloud.google.com/datastream/docs/quotas) *, which impact our use case. 


% \subsubsection{ETL on Streaming Data}
% % This ETL service provides automated data disaggregation, key-based partitioning and GZIP/ZIP/Snappy compression , all of which are beneficial for our use-case. Other considerations are that whilst multiple data destinations are available, only S3 would be appropriate for SDS-Inf; with dynamic partitioning enabled, the minimum buffer-size to trigger a write is 64MB, which is too high for us; and that SDS-Inf worker processes would still need to retrieve the data from S3, as it is not possible to directly poll/read from KDF.

% Extract transform load (ETL) solutions on streaming data offer another type of communication channel. Transformation features offered include data disaggregation and filtering, key-based partitioning and data compression, all of which would be beneficial for our use case. However, current commercial offerings (e.g., AWS Kinesis Data Firehose) have large minimum buffer sizes (both in terms of data volume and time triggers), and are not directly pollable by consumers. Hence for our use case, while producers could directly publish messages to the ETL delivery stream, the buffered output would need to be written to an intermediate destination such as object storage, from where FaaS consumers could then retrieve it.


\subsubsection{NoSQL Databases}
%DynamoDB is a low latency, high throughput NoSQL data store, which provides a serverless, on-demand capacity mode option.  Considerations for our use-case are that the maximum item (record) size is 400KB, batch update operations are not available, and that the service can be expensive for high throughput applications.
NoSQL databases typically offer low latency and high scalability (often auto-scaling based on read and write throughput). Several design options could be developed for an ML inference workload, including the maintenance of a `global' intermediate output vector/matrix, as well as a message passing approach. Some drawbacks of current offerings include restricted item sizes \footnote{https://docs.aws.amazon.com/amazondynamodb/latest/developerguide/ServiceQuotas.html} \footnote{https://learn.microsoft.com/en-us/azure/cosmos-db/concepts-limits}, limited batch update functionality, and relatively high cost compared to other communication offerings.
% described in this section.

\subsubsection{Publish-Subscribe}
%SNS provides a low latency (sub 100ms) pubish/subscribe solution which can be used in conjunction with SQS to provide a message “fan-out” architecture. It caters for unlimited produces/consumers and provides service-side filtering policies. Drawbacks for our use-case include a maximum publish size of 256KB/10 messages, and support for only raw string or JSON payloads.
Publish-subscribe (pub-sub) services offer a simple communication approach in which messages are distributed from any number of producers to unlimited subscribing consumers. 
%While they have typically not been utilized for data-intensive workloads, their 
Service-side filtering policies reduce the computational load on parallel consumers, which can be particularly beneficial in resource-constrained FaaS use cases. The potential drawbacks include restrictive payload sizes and formatting requirements, and a lack of support for direct polling of the message sinks by consumers. 

\subsubsection{Message Queues}
%SQS is a low-latency (sub 100ms) message queueing solution which offers batch enqueue and dequeue functionality and adjustable polling settings to cater for varying message arrival rates. Like SNS, drawbacks include an upper limit of 10 messages/256KB for both enqueues and dequeues, and inflexible payload types.
Cloud-based message queues offer low latency and cost-effective (batch) enqueue and dequeue functionality, as well as adjustable polling settings to cater for varying message arrival rates and consumer concurrency levels. They can also act as a destination for publish-subscribe services in a `fan-out' design. However, they typically impose similar constraints on message payloads and formats as publish-subscribe services, and lack their own service-side filtering capabilities.


\subsubsection{Object Storage}
%S3 offers a range of object storage solutions/tiers. It can scale to very high aggregate throughput when used in conjunction with multiple concurrent writers/readers. It offers virtually unrestricted object sizes and flexible content types. Drawbacks for SDS-Inf are that S3 is not specifically targetted as an inter-process communication solution, so the required functionality needs to be provided by the application. Also, certain API requests can prove expensive when used at high rates.
Object storage offers immutable and highly scalable repositories catering for very large individual file sizes. They have been shown to provide high aggregate throughput, when used in conjunction with parallel FaaS instances ~\cite{Jonas2017Occupy}. However, object storage is not specifically targeted as an inter-process communication solution, so the required functionality needs to be provided by the application. Further, object storage API calls can be expensive (up to 1 order-of-magnitude (OOM) more than equivalents in publish-subscribe/queuing offerings \footnote{https://aws.amazon.com/sns/pricing/} \footnote{https://aws.amazon.com/sqs/pricing/} \footnote{https://aws.amazon.com/s3/pricing/}). 

%---------------------------------------------------------------------------------------------------------
\input{tables/communication-channels-table}
%---------------------------------------------------------------------------------------------------------

\subsection{Hypergraph Partitioning and Parallel Computation}
\label{ss:hgp}
Since serverless functions are constrained in terms of memory and compute, we need to partition large ML models across FaaS workers, splitting the trained model weights between multiple invocations, while minimizing and balancing the communication volume. 
% An example of this for traditional MPI systems is multi-phase fixed-vertex partitioning approaches \cite{Demirci2021}. 
Multi-phase fixed-vertex partitioning approaches \cite{Demirci2021} exemplify this for traditional MPI systems.
We adapt them in this new context of FaaS-based serverless ML inference.  

The partitioning process consists of $L$ phases $\phi^k$ for $k=1,2,\dots, L$. In each phase $\phi^k$, rows of weight matrix $W^k$ (for layer $k$) are partitioned into $P$ parts. 
% , where $P$ is the number of FaaS workers we employ for the inference workload. 
For each phase $\phi^k$, a hypergraph $H(\phi^k) = (V^k \cup F^k, N^k)$ is defined, where for each matrix row $W^k(i,:)$, there exists a single vertex $v_i \in V^k$, and for each column $W^k(:,j)$ there exists a single fixed vertex $v^f_j \in F^k$ and one net $n_j \in N^k$.

% A P-way partitioning ...
A $P$-way partitioning $\Pi_P(\phi^k)=\{ V_1^k, V_2^k, \dots, V_P^k\}$ on hypergraph $H(\phi^k)$ denotes that all computational tasks corresponding to vertices in part $V_m^k \in \Pi_P(\phi^k)$ are allocated to FaaS worker $P_m$. For example, if vertex $v_i$ is assigned to part $V_m^k$, then worker $P_m$ stores row $W^k(i,:)$ and performs all computation associated with this row.

% In order to satisfy...
In order to satisfy input-output dependencies between successive layers, each net $n_j \in N^k$ connects only one fixed vertex $v_j^f \in F^k$, and fixed vertex $v_j^f$ only connects $n_j$. Fixed vertex $v_j^f$ corresponds to nonzero entry $x^{k-1}(j)$, and is fixed to the same part (and thus, worker) to which weight matrix row $W^{k-1}(j,:)$ was assigned in the previous phase $\phi^{k-1}$. This is because $x^{k-1}(j)$ is locally computed by that worker in layer $k-1$ ($v_j \in V_m^{k-1} \Rightarrow v^f_j \in V^k_m$). More intuitively, fixed vertex $v^f_j \in F^k$ ensures that after partitioning in phase $\phi^k$, net $n_j \in N^k$ connects the part/worker which is responsible for computing nonzero entry $x^{k-1}(j)$.

We partition pre-trained DNN models, and write the parts for a given worker $P_m$ over all phases, i.e. $\{V^1_m, V^2_m, \dots, V^L_m\}$, to a single file in object storage. Upon invocation, FaaS worker $P_m$ first fetches this file and loads its partition of the model weights into memory, as well as its per-layer send and receive maps. In each layer, FaaS workers consult these maps to efficiently identify and extract the subset of rows of $x^{k-1}$ they must share with each of their targets. These rows are then sent using our fully serverless communication channels. Similarly, following local computation, each worker invocation waits to receive the necessary rows from each of its sources before performing secondary computation. 

% OLD SQS FIGURE
% \begin{figure*}[h!]
% \centering
% \includegraphics[width=0.65\textwidth,height=9cm]{communication_diagram.png}
% \caption{Diagram of serverless sparse point-to-point communication scheme. Each Lambda worker has its own SQS queue pre-created (at no cost). Workers publish messages to a shared SNS topic, which forwards them to the relevant queue. Queues are polled by the workers during serverless SpFF algorithm to receive messages.}
% %\vspace{-6mm}
% \label{fig:communication-diagram}
% \end{figure*}



% \subsection{OLD Stuff}
% Commented out.
% % The proposed serverless sparse DNN inference solution is implemented on AWS. This cloud platform was selected due to the wide range of relevant services available, as well as the performance superiority of AWS Lambda compared to Google Cloud Functions and Azure Functions, particularly in cold start times [cite]. 

% % AWS does not offer a direct communication solution between Lambda function invocations, analogous to MPI in the HPC space. Existing research [cite] has tended to use S3 (AWS’s distributed object storage solution) as a communication medium between Lambda workers, where each worker reads and writes a set of files from/to S3. Limitations of this approach include high tail latency (which can lead to straggling requests), immutability of object storage, and restrictions on the number of S3 buckets per account. Other such AWS services which could be used to design a communication scheme include:

% % \begin{itemize}
% %     \item DynamoDB (NoSQL In-Memory Store): Fast for individual requests, but expensive, and does not currently offer batch update functionality (besides the use of transactions, which has further limitations).
% %     \item Kinesis Data Streams (Streaming Data Service): Since each streaming shard is limited to 5 read transactions per second, we need to create many shards to efficiently support even a moderate number of Lambda workers (since AWS recommends only using 2-3 consumers per shard). This not only adds cost, but also worker-side complexity, since for each message, the worker would have to find the appropriate partition key to ensure the message reaches the correct shard. Next, data is sent as a blob, and there is no service-side message filtering. Further, this offering is not fully serverless (even the “serverless” version does not scale down to zero).
% %     \item Kinesis Data Firehose (Streaming ETL Service): Offers automated disaggegation and partitioning by key, which would both be highly beneficial for this use case. However, the minimum buffer flush timeout is currently 60 seconds / 64 MiB, both of which are far too large for our use case.
% % \end{itemize}






==> old/3-sds-inf-architecture.tex <==
\section{SDS-Inf Architecture}
\label{s:sds-inf}



% SDS-Inf (Serverless Distributed Sparse Inference) is a fully serverless system for sparse deep neural network (DNN) batch inference. %As discussed in section \ref{s:communication}, the solution has been implemented using AWS services. 
% It consists of four core elements: serverless sparse point-to-point communication, a coordinated FaaS compute architecture, serverless algorithms for parallel sparse DNN inference, and a partitioning scheme to evenly divide computational load among resource-constrained and time-limited FaaS instances.

% SDS-Inf (Serverless Distributed Sparse Inference) is a fully serverless system for sparse deep neural network (DNN) inference. It consists of several novel core elements, including serverless sparse point-to-point communication, a coordinated FaaS compute architecture, and serverless algorithms for parallel sparse DNN inference. It also leverages hypergraph partitioning to evenly divide computational load among resource-constrained and time-limited FaaS instances.

SDS-Inf (\underline{S}erverless \underline{D}istributed \underline{S}parse Inference) is the first fully serverless system for parallel and distributed sparse deep neural network (DNN) inference. It consists of several core elements each with novel contributions. One of the main challenges is the efficient 
% communication and 
parallelization of fully-connected layers across multiple FaaS instances, due to the large communication requirements and lack of direct FaaS-to-FaaS connectivity. We therefore introduce two fully serverless sparse point-to-point data communication solutions for the cloud. % and further optimize their performance via model and data parallelism. 
The overall solution mitigates the constraints of FaaS and achieves scalable performance for ML inference at low cost, maintaining its high performance also under sporadic workloads.



\subsection{Serverless IPC Channels}

To support distributed serverless inference workloads, an ideal inter-instance cloud data communication channel should have the following properties:

\begin{itemize}
    \item Serverless (i.e. elasticity, pay-as-you-use, rapid automatic scale up/down)
    \item Low latency and high aggregate throughput
    \item Cost effectiveness
    \item Flexible payload type and message size
    \item Scalable to many concurrent producers and consumers
    \item Service-side message filtering
    \item Direct access to messages for consumers
\end{itemize}


%---------------------------------------------------------------------------------------------------------
\input{figs/fig-overall-architecture}
%---------------------------------------------------------------------------------------------------------

Table \ref{tab:comm-channels} illustrates that out of the available offerings described in Section ~\ref{ss:serverless-communication-offerings}, the categories most suitable for our problem are \textbf{publish-subscribe (pub-sub) in conjunction with message queues}, and \textbf{object storage}. 
% While none of the available offerings described in Section ~\ref{ss:serverless-communication-offerings} meet all of the above requirements, the particular categories that can potentially be adopted for our problem are \textbf{publish-subscribe in conjunction with message queues}, and \textbf{object storage}.
They are both fully serverless, with rapid scale up and down, and no \textit{`hangover’ costs} in terms of slow scaling down of burst-provisioned capacity units. Streaming ETL solutions do not offer \textit{direct polling} of the delivery stream, which adds an additional latency overhead as data must instead be written to/read from an intermediate location. We also seek flexibility of FaaS parallelism without requiring reconfiguration of communication resources. Both publish-subscribe/message queues and object storage can support this objective. On the other hand, data streaming offerings can be restrictive in terms of the \textit{numbers of producers/consumers allowed per on-demand provisioned resource}, and in time lag when auto-scaling these resources. In the compute-limited FaaS setting, \textit{service-side message filtering} is beneficial, as it reduces the computational load on parallel workers. Suitably configured pub-sub/queueing resources provide this, and a similar effect can be achieved through the careful design of an object storage solution. 



% ------------------------------------------------

% - All of the categories have a target audience; none of them aim to support FaaS-to-FaaS comm for data-intensive FaaS applications.
% - To further enhance serverless inference performance, a cloud provider could create a new service, with this use case in mind.
% - Flexibility of message payload formats and size is an important feature. If a large variety of message formats can be supported, then processing time currently spent on converting to/from restrictive data types could be saved. This would also allow for e.g. bespoke compression schemes, optimized for the vectors/matrices being used.
% - An alternative FaaS offering could also be introduced, with data-intensive processing in mind. Such a service could support e.g. GPU, longer runtime, etc, perhaps at the expense of some of the elasticity of Firecracker containers,etc.
% - Further, cloud providers could offer (perhaps) at increased cost the ability to invoke a number of co-located FaaS instances, all residing on the same machine. In this scenario, providers could relax some of the restrictions on external connectivity to FaaS containers, enabling these instances to communicate efficiently via e.g. shared memory. Distributed ML applications could then be built on top of these "FaaS clusters", possibly multiple of them, to greatly improve performance.

% Floki (kubernetes)
% Boxer (NAT hole punching)




In the context of serverless ML inference, we examine the trade-off between the lower cost but payload-restrictive messaging supported by pub-sub/queueing based solutions, with the more expensive but effectively size-independent data transfers possible when using object storage.

\subsection{SDS-Inf Overview}

Our solution is cloud-provider agnostic. In light of AWS Lambda’s short `cold start' time and relatively long maximum runtime (15 minutes) ~\cite{Rifai2021}, we develop the design principles of SDS-Inf on AWS Lambda. Hence, we also adapt AWS services for inter-process communication channels; namely, Simple Notification Service (SNS) and Simple Queue Service (SQS) for pub-sub/queueing, and Simple Storage Service (S3) for object storage. We characterize SDS-Inf with these two communication approaches as \textbf{SDS-Inf-Queue} and \textbf{SDS-Inf-Object}, respectively. It should be stressed that equivalent solutions could readily be built on other cloud platforms. Note that we also consider the use of SDS-Inf with a single worker with no communication components; we term this variant \textbf{SDS-Inf-Serial}.



% Our work leverages techniques proposed for sparse distributed inference in \cite{Demirci2021}, and translates them into a fully serverless cloud-based setting. The compute component is an AWS Lambda “worker” function which concurrently executes the Serverless SpFF (Sparse FeedForward) algorithm discussed below. Multiple function instances are invoked hierarchically to minimise cold-start delay. 

% Figure \ref{fig:overall-architecture} displays the high-level architecture of SDS-Inf. Each Lambda worker begins by reading its model weights, inference data and connectivity data from S3. It then executes the Serverless SpFF algorithm presented in algorithms \ref{alg:spff-sns} and \ref{alg:spff-s3}. In each algorithm, workers carry out sparse point-to-point communication using one of the two fully serverless communication channels described below.



Figure \ref{fig:overall-architecture} displays the high-level architecture of SDS-Inf. Upon invocation, each FaaS instance reads its share of the model weights, inference data and per-layer send and receive maps. 
%The hypergraph partitioning scheme outlined in Section ~\ref{ss:hgp} is employed to b
% A balanced computational load is assigned to each parallel FaaS instance, whilst minimizing the overall data volume sent over the serverless communication channels.
Each worker then executes the Serverless SSpInf routines presented in Algorithms \ref{alg:sspinf-queue} (SDS-Inf-Queue) and \ref{alg:sspinf-object} (SDS-Inf-Object).
% The sparse point-to-point communication in each algorithm ensures that workers send and receive only the necessary rows to perform the distributed SpMV/SpMM in each layer.
% We achieve model 
The proposed highly parallel approach, with its efficient communication mechanisms, is shown to mitigate the inherent constraints of FaaS for a scalable serverless solution.  
% Once all workers have completed their processing for the final layer of the model, a reduce operation is performed, and the root worker returns the overall inference result.




%---------------------------------------------------------------------------------------------------------
\input{figs/fig-comm-queues}
%---------------------------------------------------------------------------------------------------------



% \subsection{SNS, SQS and DynamoDB Communication Scheme}
\subsection{SDS-Inf-Queue Communication Channel}
\label{ss:sds-inf-queue}


% Prior to runtime we pre-create two SNS topics (one for data and one for per-batch synchronisation), and as many SQS queues as the maximum number of workers we may be deploying ($P$). There is no limit on the number of queues per AWS account, and no cost for the passive existence of each queue. We then create SNS subscriptions between each of these queues and both SNS topics. Onto each subscription to the data topic, we add a filter policy such that only messages with a single value of message attribute “sourceWorkerID” are forwarded to the subscribing queue by the SNS service. Such a filter policy is not required for the synchronisation topic, as all-to-all communication is required at this stage.



% Under this scheme, each worker only publishes messages to these two SNS topics, rather than having to make individual connections to each target queue. The backend SNS service handles the distribution of messages to the relevant queues (and in turn, the relevant workers). Each worker has to poll only a single SQS queue to receive its messages (both for intermediate inference data and synchronisation), with no worker-side message filtering required. The proposed design is illustrated in figure \ref{fig:sns-comm}. We also create a DynamoDB table which is used to communicate instances when a given worker has no nonzero entries to send to a target. DynamoDB is chosen for its very low latency and cost-effectiveness for small writes/reads. Further detail on how this communication scheme is utilised for inference is provided in section (4.4).

Figure ~\ref{fig:sns-comm} illustrates the proposed SDS-Inf-Queue architecture. To design a fast and scalable serverless communication scheme for distributed ML inference, we aim to maximize the overall communication throughput, whilst avoiding I/O bottlenecks and minimizing the computational overhead on the resource-constrained FaaS instances. %; fast and scalable inter-process communication is a key requirement for any such system. 
Several design features of SDS-Inf-Queue contribute to these goals. These include parallel pub-sub topics to increase aggregate throughput and avoid potential I/O bottlenecks, and a dedicated message queue per parallel FaaS instance to minimize the number of service-to-service network connections required. This avoids the need for consumer-side message filtering (and hence the parsing/discarding of unwanted messages intended for other workers). We leverage a `fan-out’ architecture to offload the targeted distribution of messages onto the pub-sub service, helping to reduce computational overheads. Finally, we pre-create the required communication resources (pub-sub topics, queues) to avoid doing so at inference time, at no additional provisioning or ongoing cost. Further details on how this communication scheme is utilized for sparse DNN batch inference are provided in Section ~\ref{sss:pub-sub-queueing-inference-specifics}.


%---------------------------------------------------------------------------------------------------------
% \input{algos/serverless-spff-sns}
\input{algos/sds-inf-queue-algorithm}
%---------------------------------------------------------------------------------------------------------


\subsection{SDS-Inf-Object Communication Channel}
% Ahead of runtime, we create 10 S3 buckets to handle the communication of intermediate inference results between workers. Each AWS account can create up to 100 buckets. In a given layer, each worker may need to communicate with all other workers, so the maximum number of API requests is quadratic in $P$. The current rate limits are 3.5k and 5.5k per second per prefix for writes and reads respectively (todo: link to docs in footnote); this can easily be exceeded for large worker counts. As a simple workaround, we use 10 buckets for this data exchange, effectively increasing the API request limit tenfold. Modular arithmetic determines which bucket each worker should write to for a given target. The proposed design is presented in figure \ref{fig:s3-comm}. Further detail on how data is sent and received using S3 is given in section (4.4).

As in SDS-Inf-Queue, our key objectives are to maximize aggregate communication throughput at minimal computational effort for FaaS workers. In SDS-Inf-Object, we employ multiple object containers and prefixes for the intermediate results files. This helps avoid I/O bottlenecks, whilst staying within provider-imposed API quotas\footnote{https://docs.aws.amazon.com/AmazonS3/latest/userguide/optimizing-performance.html}; in object storage solutions such as S3, using $k$ containers effectively increases the API request limit $k$-fold \cite{Muller2020Lambada}. Under this design, each worker only needs to scan/read from a single object storage container name and file prefix. The unnecessary reading of empty files (i.e. where a source had no information to transmit to a target in the current layer) is avoided by the use of distinct suffixes for empty/non-empty files. We also initiate object storage read operations in multiple parallel threads per worker, to minimize delays between folder scans. Figure ~\ref{fig:s3-comm} presents the proposed SDS-Inf-Object architecture, and Section ~\ref{sss:object-storage-inference-specifics} provides further details on its use for sparse DNN batch inference.



%---------------------------------------------------------------------------------------------------------
\input{figs/fig-comm-s3}
%---------------------------------------------------------------------------------------------------------


%---------------------------------------------------------------------------------------------------------
% \input{algos/serverless-spff-s3}
\input{algos/sds-inf-object-algorithm}
%---------------------------------------------------------------------------------------------------------


\subsection{SSpInf Algorithm}
\label{ss:serverless-spff}




% As in \cite{Demirci2021}, our Serverless SpFF algorithm performs repeated distributed SpMV in the form of $W^kx^{k-1}$ for each layer $K=1,2,\dots,L$. Model parallelism is achieved through the row-wise hypergraph partitioning of weight matrices $W^k$ and input/output vectors $x^{k-1}$ described in section \ref{ss:hgp}.

We propose two serverless SSpInf (Serverless Sparse Inference) algorithms, each performing repeated distributed SpMV (for single sample inference) / SpMM (for batch inference) in the form of $W^kx^{k-1}$  / $W^kX^{k-1}$ for each layer $k=1,2,\dots,L$. We will henceforth present notation for SpMV, but this should be understood as also applying to SpMM. Models are parallelized through the row-wise hypergraph partitioning of sparse weight matrices $W^k$ and input/output vectors $x^{k-1}$. 


% Algorithms \ref{alg:spff-sns} and \ref{alg:spff-s3} describe the execution of the Serverless SpFF algorithm using the SNS/SQS and S3 communication channels, respectively. In both algorithms, each processor $P_m$ for $m = 1, 2, \dots, P$ holds row-blocks $W^k_m$ and $x^{k-1}_m$ of $W^k$ and $x^{k-1}$ respectively. The offline hypergraph partitioning scheme also provides each processor $P_m$ with maps $Xsend_m^k$ and $Xrecv_m^k$ respectively which map row indices of $x^{k-1}_m$ to be communicated with target/source processor IDs. These are implemented using SciPy \texttt{csc\_matrix} for efficient column access. As in \cite{Demirci2021}, these sets are formally defined as:

Algorithms \ref{alg:sspinf-queue} and \ref{alg:sspinf-object} describe the execution of the serverless SSpInf routine using the pub-sub/queueing (SDS-Inf-Queue) and object storage (SDS-Inf-Object) communication channels, respectively. In both algorithms, each FaaS processor $P_m$ for $m = 1, 2, \dots, P$ holds row-blocks $W^k_m$ and $x^{k-1}_m$ of $W^k$ and $x^{k-1}$ respectively. The hypergraph partitioning scheme also provides each processor $P_m$ with maps $Xsend_m^k$ and $Xrecv_m^k$ which match row indices of $x^{k-1}_m$ to target/source worker IDs with which they should be shared \cite{Demirci2021}. These sets are formally defined as:
\begin{equation}
Xsend_m^k = \bigl\{ (P_n, \bar{x}_{mn}^{k-1}) |  \bar{x}_{mn}^{k-1} = x^{k-1}_m[cols(W^k_n) \cap rows(W^{k-1}_m)] \bigr\}
\label{eqn:xsend}
% \vspace{-1mm}
\end{equation} 

\begin{equation}
Xrecv_m^k = \bigl\{ (P_n, \hat{x}_{nm}^{k-1}) | \hat{x}_{nm}^{k-1} = x^{k-1}_n[cols(W^k_m) \cap rows(W^{k-1}_n)] \bigr\}
\label{eqn:xrecv}
% \vspace{-1mm}
\end{equation} 

As shown in Equations \ref{eqn:xsend} and \ref{eqn:xrecv}, in order to perform SpMV $W^k_mx^{k-1}_m$, worker $P_m$ must receive all rows of $x^{k-1}$ corresponding to the indices of the nonzero weight matrix columns it holds for layer $k$ (i.e. $cols(W^k_m))$, from the workers which manage these rows. 

% Prior to performing non-blocking sends (line 7 in Algorithm ~\ref{alg:spff-sns}, lines 5/8 in Algorithm ~\ref{alg:spff-s3}), each worker first iterates through tuples $(P_n, \bar{x}^{k-1}_{mn})$ in its send map for the current layer. For each row in $\bar{x}^{k-1}_{mn}$, we determine if $P_m$ has any nonzero entries for that row. We maintain two sublists of row indices in $\bar{x}^{k-1}_{mn}$, indicating for which rows $P_m$ has nonzero entries and for which rows it does not.

The mechanism for sending and receiving intermediate results using SDS-Inf-Queue and SDS-Inf-Object is as follows:

\subsubsection{SSpInf with SDS-Inf-Queue}
\label{sss:pub-sub-queueing-inference-specifics}
% Commented 05/06/2023
% If it is determined that $P_m$ holds no nonzero entries in any of the rows to be communicated to $P_n$ in layer $k$, we write a record $((k, n), m)$ to a shared NoSQL table which, when polled by $P_n$, indicates that it can discard $P_m$ as a data source for layer $k$. We utilize a NoSQL table here as a low latency flagging mechanism, and because these writes are few in number and minimal in size we avoid the high cost associated with a NoSQL-only communication solution.

% If $P_m$ does have rows containing nonzero entries to send to $P_n$, we then construct messages to publish to SNS. Due to the requirements of SNS/SQS, these messages take the form of byte strings, representing compressed SciPy \texttt{COO} matrices (\texttt{COO} chosen for ease of reconstruction). As the maximum size of an SNS message is 256KB, we use the total NNZ across the rows to be communicated to estimate the number of byte strings required to encode $\bar{x}^{k-1}_{mn}$; this list of byte strings is denoted as $\{\bar{x}^{k-1}_{mni}\}$. All byte strings are added to $Xsend\_list^k_m$, from which we populate a series of message batches (this process is multi-threaded in each worker). Note that we also add several message attributes, including the source worker ID (used for server-side message filtering), the total number of byte strings to be sent to this target (used by the target to determine when it has received all incoming data from this source), and the message layer (it is possible that the source is in a later layer than the target; we enable the source to safely “pre-receive” data for a layer it is yet to reach). %(Omitting coord attribute because it isn’t very interesting)

For each target $P_n$ that source worker $P_m$ must communicate with in a given layer, we construct messages to send to a pub-sub topic. Due to the current provider-imposed constraints of the cloud pub-sub service, these messages consist of size-limited byte strings, representing compressed sparse matrices. We use the total number-of-nonzeros (NNZ), over the rows to be communicated, as an experimentally-determined heuristic to estimate the number of byte strings required to encode $\bar{x}^{k-1}_{mn}$. This list of byte strings is denoted as $\{\bar{x}^{k-1}_{mni}\}$. The goal of this process is to maximize the utilization of the allowed pub-sub message payload size, whilst grouping and compressing rows only once.

All byte strings are added to a send buffer $Xsend\_list^k_m$, from which we populate a series of message batches (to minimize API calls and hence cost); this process is multi-threaded in each worker. Note that we also add several message attributes, including the source worker ID (used for service-side message distribution), the total number of byte strings to be sent to this target (used by the target to determine when it has received all incoming data from this source), and the message layer (as it is possible that the source is in a later layer than the target). %(Omitting coord attribute because it isn’t very interesting)

%------------------------------------------------------------------------------------------------------------------------------------------------


% These message batches are used as input to \texttt{SNS.publish\_batch()}, and contain either up to 10 messages, or 256KB of data, (as per current SNS/SQS message size limits). We then asynchronously publish the message batches to SNS, which distributes it to each target’s SQS queue using a subscription filter policy. In order to overlap communication with computation, we then perform local SpMV computation $z^k_m = W^k_mx^{k-1}_m$, before receiving any $x^{k-1}$ rows from other processors.

Having constructed these message batches (which are limited in terms of number of messages and total size\footnote{https://docs.aws.amazon.com/general/latest/gr/sns.html}), we then use parallel threads to issue them to the pub-sub topic, which distributes them to each target's dedicated message queue using a filter policy. In order to overlap communication with computation, we then perform local SpMV $z^k_m = W^k_mx^{k-1}_m$, before receiving any $x^{k-1}$ rows from other workers, hence helping to amortize communication overheads.



%------------------------------------------------------------------------------------------------------------------------------------------------


% When receiving messages from other workers (lines 11-18), worker $P_m$ repeatedly polls the communication channel until all the data in $Xrecv_m^k$ has been received. We first query the DynamoDB table for null message flags for $P_m$ in layer $k$, removing any sources $P_n$ that are returned from $Xrecv_m^k$. We then poll the SQS queue using long polling. 


In order to receive messages from other workers (lines 9 to 15 in Algorithm~\ref{alg:sspinf-queue}), worker $P_m$ repeatedly polls the SDS-Inf-Queue communication channel until all rows in $Xrecv_m^k$ have been obtained. We poll the message queue using `long' polling. In the case of the AWS message queueing solution, the user can choose between `long' and `short' polling by setting a parameter henceforth referred to as $W$. `Short' polling ($W=0$) polls the queue, and responds immediately regardless of whether messages were found. It should be noted that the message queueing service distributes messages over multiple servers (outside of user control); it is possible when performing `short' polling that not all servers are queried, and thus messages may be missed by a given request. With `long' polling ($W > 0$), all servers are guaranteed to be queried. As soon as messages are found, they will immediately be returned. If messages are not immediately found, the service will wait for up to $W$ seconds (still continuously checking for messages without incurring additional request costs), and can only return empty-handed after this period has elapsed. Our experimental analysis confirms that long polling outperforms short polling, and enables significantly more messages to be returned per poll request (reducing costs). 



%------------------------------------------------------------------------------------------------------------------------------------------------



% SQS enables the user to choose between long and short polling by setting parameter \texttt{WAIT\_TIME\_SECS}, henceforth referred to as $W$. Short polling ($W == 0$) polls the queue, and immediately returns if no messages are found. It should be noted that the SQS service distributes (without user control) messages over multiple servers; it is possible when performing short polling that not all servers are queried, and thus messages may be missed by a given request. With long polling ($W > 0$), all servers are guaranteed to be queried. As soon as messages are found, they will immediately be returned. If messages are not immediately found, the SQS service will wait for $W$ seconds (still continuously checking for messages without incurring additional request costs), and can only return empty-handed after this period has elapsed. We found that long polling outperformed short polling, enabled significantly more messages to be returned per poll request (saving costs). %Additionally, the user can specify the \texttt{VISIBILITY_TIMEOUT}, i.e. the period for messages to remain hidden from other requests having been observed. Since only one worker is ever polling each queue, this is not a factor in SDS-Inf.




%Additionally, the user can specify the \texttt{VISIBILITY_TIMEOUT}, i.e. the period for messages to remain hidden from other requests having been observed. Since only one worker is ever polling each queue, this is not a factor in SDS-Inf.




%------------------------------------------------------------------------------------------------------------------------------------------------



% For each byte string returned in the poll, we examine its message attributes to determine which source it is from, and which layer it pertains to. The deserialised and decompressed message body is added to $Xrecv\_list_{m}^k$. If all the expected byte strings from source ID $n$ has been received (determined by the message attributes described above), we remove worker $n$ from $Xrecv_m^k$.


For each message returned in the poll, we add its deserialized and decompressed body to $Xrecv\_list_{m}^k$. We cater for the case where source $P_n$ needs to send multiple messages to target $P_m$ using message attributes, and only remove worker $P_n$ from $Xrecv_m^k$ when all its expected byte strings for layer $k$ have been received.



%------------------------------------------------------------------------------------------------------------------------------------------------


\subsubsection{SSpInf with SDS-Inf-Object}
\label{sss:object-storage-inference-specifics}
% Due to the large 5TB maximum S3 file size, each worker will only need to write a single file to S3 for each of its targets in a given layer. This is in contrast to the 256KB message size limit experienced in SNS/SQS. Under this scheme, worker $m$ sending intermediate inference results to worker $n$ in layer $k$ would write a file named as:

Due to the large file sizes available with object storage solutions, each FaaS instance in SDS-Inf-Object only needs to write a single object for each of its targets in a given layer. In contrast, SDS-Inf-Queue experiences far more constrained message sizes. As an illustration, at present SDS-Inf-Queue has a 256KB limit, whilst we send single objects of up to 29MB with SDS-Inf-Object, resulting in significantly fewer API calls (though it should be noted that object storage API calls are more costly). 
Prior to performing non-blocking sends (lines 5/8 in Algorithm~\ref{alg:sspinf-object}), each worker first iterates through tuples $(P_n, \bar{x}^{k-1}_{mn})$ in its send map for the current layer. For each row in $\bar{x}^{k-1}_{mn}$, we determine if $P_m$ has any nonzero entries for that row. We maintain two sublists of row indices in $\bar{x}^{k-1}_{mn}$, indicating for which rows $P_m$ has nonzero entries and for which rows it does not.
Under SDS-Inf-Object, worker $P_m$ sending intermediate inference results to worker $P_n$ in layer $k$ would write a file named:

\texttt{“s3://bucket-\{n\%10\}/\{k\}/\{n\}/\{m\_n\}.dat”}.

When worker $m$ has no nonzero entries to communicate to worker $n$ in layer $k$, it will instead write a 0-bytes file:

\texttt{“s3://bucket-\{n\%10\}/\{k\}/\{n\}/\{m\_n\}.nul"}

%------------------------------------------------------------------------------------------------------------------------------------------------
% This is instead of the DynamoDB table used in the previous communication scheme for null messages; workers do not perform a \texttt{get\_object()} request on files with this extension.  We also maintain an S3 lifecycle policy to delete this ephemeral data 1 day after use, in order to reduce costs. 

Workers do not attempt to retrieve files with the \texttt{".nul"} extension when they are identified in folder scans. 

%------------------------------------------------------------------------------------------------------------------------------------------------

% When looking to receive data from other workers, a worker will repeatedly list the files in the bucket/prefix “bucket-\{m\%10\}/k/m/”. For all of the file names \texttt{\{n\_m\}.\{suffix\}} returned, we first check the suffix; if it is ".nul", we can safely remove $(P_n, \hat{x}^{k-1}_{nm})$ from $Xrecv^k_m$. Any ".dat" files addressed from sources $P_n$ that have already been processed are ignored. The remaining ".dat" files are then read into memory using \texttt{S3.get\_object()}, decompressed and added to $Xrecv\_list^k_m$.

In order to retrieve data sent by source FaaS instances, a worker will repeatedly scan the files in the location “\texttt{bucket-\{m\%10\}/k/m/”}. For all file names \texttt{\{n\_m\}.\{suffix\}} identified by the scan, we remove $(P_n, \hat{x}^{k-1}_{nm})$ from $Xrecv^k_m$ for files ending \texttt{".nul"}. Any \texttt{".dat"} files from sources $P_n$ where $(P_n, \hat{x}^{k-1}_{nm}) \notin Xrecv^k_m$ are ignored, as data from $P_n$ has already been received. The remaining \texttt{".dat"} files are then read into memory, decompressed and added to $Xrecv\_list^k_m$.

%------------------------------------------------------------------------------------------------------------------------------------------------

\subsubsection{Post-Communication Processing}
Once data from all the row indices in $Xrecv_m^k$ is stored in $Xrecv\_list_m^k$, we iterate through each sparse matrix $\hat{x}^{k-1}_{nm} \in Xrecv\_list_m^k$ and perform operation $z^k_m \gets z^k_m + W^k_m\hat{x}^{k-1}_{nm}$, to complete the distributed SpMV for layer $k$. The final operation in each layer is the application of an activation function $f(\cdot)$.

After layer $L$, we perform barrier and reduce operations to synchronize all workers, and communicate all output vectors $x^L_m$ to worker $P_0$, respectively. $P_0$ then aggregates them to calculate the overall inference result $x^L$. This entire process can then be repeated across multiple successive inference samples/batches.



% \input{4.5-lambda-invocation}



==> old5-related-work.tex <==
\section{Related Work}
\label{s:related-work}
% Two research areas are particularly relevant to SDS-Inf.
% The first is the application of serverless computing for data analytics and machine learning (ML) tasks, and the second covers the use case of sparse deep neural network (DNN) inference.

\subsection{Serverless Computing}
\label{ss:related-work-serverless-overview}

% \subsubsection{Applications of Serverless Computing}
In recent years there has been increasing exploitation of cloud-based serverless solutions for different types of computing workloads~\cite{Shafiei2022, Schleier-Smith2021, Khandelwal2020Taureau, ServerlessSurvey2022}. 
% The growing ecosystem of serverless services (storage, DBMS, messaging, streaming, etc.) is key to this trend, and cloud providers have invested heavily in this area. 
It is now possible to build a range of cloud-based applications using only serverless, pay-as-you-go/pay-for-what-you-use offerings. Starting with relatively simple functionality such as web backends and IoT consolidation, the range of potential use cases has continued to evolve and now extends to data management and analytics~\cite{Muller2020Lambada, Perron2020}, DBMS/DBaaS~\cite{Li2022DBaaS}, linear algebra~\cite{Shankar2020NumPyWrenSLA}, ML inference~\cite{Ishakian2018, Jarachanthan2021AMPS}, ML training~\cite{Jiang2021Demystifying} and end-to-end ML pipelines~\cite{Paraskevoulakou2021}.

\subsubsection{Mitigating Serverless Constraints}
Recent work addresses some of the challenges arising from the use of serverless architectures for data-intensive applications. 
% Flint ~\cite{Kim2018Flint}, Corral ~\cite{Congdon2018Corral} and Qubole ~\cite{Sowrirajan2017Qubole} are AWS Lambda-based implementations of PySpark, MapReduce and Spark respectively. 
Methods are proposed~\cite{Daw2020Xanadu, Carver2019DAG, Carver2020WukongNew, Icebreaker2022} for quickly launching large numbers of function instances while reducing the `cold-start' overhead this can entail, for example by pre-analyzing task chains and pre-launching resource instances to reduce start-up delays. 
Gupta et al.~\cite{ReliableTransactionsICDE2023} address the integration of edge devices with multi-cloud FaaS instances and secure data stores in a fault-tolerant manner.
AsyFunc~\cite{AsyFunc2023} considers the impact of bursty workloads in a serverless inference environment and proposes offloading resource-sensitive layers to `shadow function' instances which co-operate and synchronize with full-model instances.
% Other works seek to predict pause/resume patterns in serverless cloud DBMS workloads to minimize delays after idle periods ~\cite{Poppe2022Moneyball}, and to predict peak parallelism levels for big data analytics queries ~\cite{Sen2020AutoToken}. 
Several benchmarks are proposed to analyze characteristics of serverless platforms~\cite{Yu2020Benchmark1, Kim2019Benchmark2}.
The issue of `straggler' worker instances is also addressed by various methods including pre-emptive read/write retries~\cite{Perron2020} and by the use of local error-correcting codes~\cite{Gupta2020StragglerLocalErrorCorrecting, Bartan2019StragglerPolar}. Several studies consider how best to design systems which unify serverless and serverful components~\cite{GarciaLopezServerMix2019, Suresh2021ServerMore}. The lack of direct instance-to-instance communication capabilities in the serverless environment is a key challenge. 
% Improvements to Azure Durable Functions (DFs) for message passing models are explored ~\cite{Burckhardt2022Netherite}. 
A NAT `hole-punching' approach is proposed~\cite{Wawrzoniak2021Boxer, Moyer2021} which enables communication between FaaS function instances via an external proxy server. This is incorporated in a wider serverless communication solution which emulates a subset of MPI functionality~\cite{Bohringer2022FMI}. Our work also implements MPI primitives (Send, Recv, Broadcast, Reduce), but avoids the use of an external provisioned server, achieving fully serverless communication.
Over recent years an ecosystem of Docker-based, Kubernetes-managed cloud compute services has also developed, with Knative and similar solutions enabling FaaS offerings to be built on top of this stack.
Such services 
%can offer additional platform independence (cloud and on-premise), freedom of choice of runtimes, programming languages and toolsets, and user-specified containers. 
%They 
are usually `scaled-by-concurrency', enabling multiple function instances on the same container which is controlled by the cloud provider, with the user specifying a concurrency target/limit. 
Providers now offer FaaS solutions based on Knative; Google Cloud Run~\cite{GoogleCloudRun} and IBM Cloud Code Engine~\cite{IBMCloudCodeEngine} are examples. 
While this is an area of fluid change, our approach can readily adapt to such emerging FaaS architectures. 

% Adopting a different perspective, %García-López \textit{et al.} 
% ~\citet{GarciaLopezServerMix2019} argue that it is difficult to mitigate the challenges presented by serverless architectures, and that optimal solutions are usually hybrids which appropriately combine serverless and server-based elements. 
% % Similarly, `gg' ~\cite{Fouladi2019} is a framework which enables developers to build and execute burst-parallel applications; its architecture includes client-side components, warm cloud-hosted VMs and FaaS functions. Crucial ~\cite{BarcelonaPonsFaasTrack} is a hybrid framework consisting of a Java-based client program, a distributed storage layer hosted on cloud-based VMs, and AWS Lambda function instances. 
% In contrast, we show that our fully serverless solution (which has no pre-provisioned elements) can indeed achieve competitive performance at low cost.

\subsubsection{Stateful Functions}
A new category of offerings incorporates `stateful functions'~\cite{Statefun, Cloudburst2020, Orleans2011, AzureDurableFunctions2021} based on elements of the Actor model~\cite{ActorModel1973}. These offer state management and function-to-function communication mechanisms. However, they typically rely on non-serverless infrastructure services and do not target a fully serverless offering.

\subsection{Serverless Data Analytics and ML}
\label{ss:related-work-serverless-da-ml}

\subsubsection{Serverless Data Analytics}


Lambada~\cite{Muller2020Lambada} presents efficient scan, sort and shuffle operations for data analytics using object storage as a communication channel. Our work enhances shuffling by incorporating both object storage and pub-sub/queueing for data communication. We also leverage hypergraph partitioning to minimize communication requirements and ensure balanced workloads across parallel workers. For pub-sub/queueing, we offload the distribution and filtering of messages to the back-end cloud service.


Other works explore the use of serverless for Linear Algebra (LA) workloads. 
PyWren~\cite{Jonas2017Occupy} is a serverless system which provides a MapReduce-style capability for a range of scientific and data analytics workloads. %PyWren spawns multiple cloud-based FaaS instances to execute the workloads, as opposed to multiple locally hosted parallel processes. 
% PyWren seeks to enable users to submit existing single-machine code, have it run in the cloud across multiple parallel function instances. %, and for consolidated results to be returned in a timely fashion. It does not attempt to equal the performance of specialist clustered platforms, but simply to provide much better performance than the user would obtain by running their application on a local workstation or server. 
NumPyWren~\cite{Shankar2020NumPyWrenSLA} leverages the PyWren framework in conjunction with LAmbdaPACK, a domain-specific language for coordinating the execution of the tasks underpinning LA algorithms. 
% It attempts to mirror implementations found in ScaLAPACK, a library with a similar purpose for use on MPI architectures. 
Unlike these works, which study dense linear algebra, we focus on scalable ML inference. We are also able to leverage sparse data structures and point-to-point communication techniques to exploit the sparsity of the underlying data, i.e. both weight matrices and input vectors. This improves computational performance while reducing IPC overheads. Further, NumPyWren~\cite{Shankar2020NumPyWrenSLA} only mimics a serverless runtime, whereas FSD-Inference truly utilizes a fully serverless architecture


\subsubsection{Serverless Machine Learning Systems}
A number of recent works consider the suitability of serverless platforms for ML workloads. 
%Whilst relatively few address serverless ML training ~\cite{Jiang2021Demystifying}, t
There has been a particular interest in serverless ML \textit{inference} use cases~\cite{Wu2021}. Park et al.~\cite{Park2022AYCI} consider optimal FaaS configurations for inference, but do not cater for per-request parallelism. 
Tetris and Photons~\cite{Tetris2022, Photons2020} adapt Kubernetes-based FaaS offerings to enable runtime and tensor sharing to reduce memory usage, whilst our work achieves this via model and data partitioning.
AWS now offers a commercial serverless inference endpoint as part of its SageMaker suite~\cite{AWSServerlessInference}. Whilst this service can scale upwards (currently to 6GB memory) and outwards (via auto-scaling in response to demand levels), it does not yet address the challenges of per-request data parallelism, or ML model parallelism, which is a requirement for very large DNNs. 
A small number of studies have attempted to combine serverless inference with model parallelism.
Gillis~\cite{Gillis2021} and AMPS-Inf~\cite{Jarachanthan2021AMPS} seek to efficiently partition trained models in a layer-wise fashion over multiple FaaS instances. They adopt `layer grouping' algorithms which co-locate layers (or segments of layers) which can be processed together without requiring substantial inter-instance communication. In contrast, our work is the first to employ \textbf{intra-layer} (i.e., tensor) model parallelism in the serverless setting, distributing consecutive fully-connected layers over multiple FaaS instances.

Another important area of interest is \textit{batch} serverless inference, as there are real-world use cases where an immediate response to an inference request is not required, and where request arrival is sporadic and/or bursty. This type of workload is a sweet-spot for serverless inference, as it can often be more cost-effective than sample-by-sample processing. BATCH includes a buffering system and a profiler/analytical model which identifies an SLO-optimal FaaS deployment (batch size, memory config) to carry out batch inference workloads~\cite{Ali2020Batch}. Ali et al.~\cite{Ali2022OptInfServ} propose a performance and cost estimator % based on analytical models and Bayesian optimization, 
to efficiently batch together heterogeneous serverless inference requests. 
Hybrid server-based/serverless batch inference solutions, which use serverless to supplement IaaS resources when handling bursty workloads, have also been proposed~\cite{Zhang2019}.
In contrast, our solution caters for batch inference processing as part of the core serverless design, although we assume that requests have been buffered and batched by an appropriate mechanism prior to FSD-Inference processing.


% \subsection{Sparse Deep Neural Network Inference}
% \cite{Kepner2019} describe how the increasing sizes of state-of-the-art DNNs has led to sparsification and pruning of DNNs via various methods
% \cite{Geng2021-O3BNN, Hassibi1992SecondOrderDerivatives, Kepner2020, LeCun1989, Liu2015, Srivastava2014}. Demirci and Ferhatosmanoglu \cite{Demirci2021} propose a hypergraph-based partitioning method for sparse DNN weights which is shown to outperform previous solutions. Algorithms and demonstrations are provided of scalable distributed DNN training and inference using model weights partitioned in this way. We adapt hypergraph partitioning to help balance the load among resource-constrained FaaS instances, and reduce the communication volume between workers. The serverless setting necessitates a parallel inference approach with a smart partitioning scheme, when handling large and deep DNNs. Without these in place, individual lightweight FaaS invocations could likely not perform inference within the restrictive maximum function runtime, and may not even be able to load the model weights (as well as dependencies, inference data, etc.) into memory. 

% % Kepner \textit{et al} \cite{Kepner2019} describe how the increasing sizes of state-of-the-art DNNs has led to a research focus on the sparsification of DNNs via various methods including Hessian-based pruning, Hebbian pruning, matrix decomposition and graph techniques. % Whilst network sparsification reduces memory requirements without significant loss of prediction accuracy compared to dense networks, it poses new challenges for the distribution of the inference workload over multiple processors, as unlike with dense networks, naïve (e.g. random) partitioning is unlikely to result in balanced workloads.






==> plots/plot-surface-1-both.tex <==
\begin{figure}[h]%[tb]%[!h]%
\centering  %
%\vspace{-3mm}
\subfloat[HGP-DNN]
% {\label{surface-1-subfloat-hgp}\includegraphics[width=0.35\textwidth]{plots/surface_1_total_rows_sent_hgp.pdf}}
{\label{surface-1-subfloat-hgp}\includegraphics[scale=0.36]{plots/surface_1_total_rows_sent_hgp.pdf}}
\\
\subfloat[RP]
% {\label{surface-1-subfloat-rp}\includegraphics[width=0.35\textwidth]{plots/surface_1_total_rows_sent_random.pdf}}
{\label{surface-1-subfloat-rp}\includegraphics[scale=0.36]{plots/surface_1_total_rows_sent_random.pdf}}
%\vspace{-2mm}
\caption{Surface plots showing total number of rows sent per layer, by each worker, for $N = 16384$, $P = 42$, under HGP-DNN and RP.}
\label{surface-1-subfloats}
%\caption{\textcolor{green}{Partition Number against different $\varepsilon_{p}$}}\label{TSPI_Example}
%\vspace{-6mm} 
\end{figure}
